Black box variational inference for state space models

Latent variable time-series models are among the most heavily used tools from machine learning and applied statistics. These models have the advantage of learning latent structure both from noisy observations and from the temporal ordering in the data, where it is assumed that meaningful correlation structure exists across time. A few highly-structured models, such as the linear dynamical system with linear-Gaussian observations, have closed-form inference procedures (e.g. the Kalman Filter), but this case is an exception to the general rule that exact posterior inference in more complex generative models is intractable. Consequently, much work in time-series modeling focuses on approximate inference procedures for one particular class of models. Here, we extend recent developments in stochastic variational inference to develop a `black-box' approximate inference technique for latent variable models with latent dynamical structure. We propose a structured Gaussian variational approximate posterior that carries the same intuition as the standard Kalman filter-smoother but, importantly, permits us to use the same inference approach to approximate the posterior of much more general, nonlinear latent variable generative models. We show that our approach recovers accurate estimates in the case of basic models with closed-form posteriors, and more interestingly performs well in comparison to variational approaches that were designed in a bespoke fashion for specific non-conjugate models.

==> texdefs.tex <==
% Standard environments here
\usepackage{mathtools} % pmatrix*! use \begin{matrix*}[r] to center colums right


% ----  Custom Environments ----- 
% just a horizontal rule for the "details" environment
\newcommand{\optionrule}{\noindent\rule{1.0\textwidth}{0.75pt}}
% the "details" environment declaration.
\newenvironment{aside}{%
  \def\FrameCommand{\hspace{2em}}
  \MakeFramed {\advance\hsize-\width \small}\optionrule}
{\\\optionrule\endMakeFramed}
% I took out the newline command. i don't know what it did.
%{\newline\optionrule\endMakeFramed}

% ---- Text/Formatting Symbols ---
\renewcommand{\eqref}[1]{eq.~\ref{eq:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
%\renewcommand{\etal}{{\it et al} }

% ---- Math symbols ------------

% basic algebra, set-theoretic, and functional notation
\newcommand{\set}[1]{\{#1\}} % set notation
\newcommand{\Range}{\mathcal{R}} % range (ie, of a function)
\newcommand{\setcomp}[1]{{#1}^{\mathsf{c}}} % set complement
%\newcommand{\inv}{^{-1}} % inverse
\newcommand{\inv}[1]{\ensuremath{{#1}^{-1}}} 
\newcommand{\ind}[1]{\mathbf{1}_{\left\{ #1\right\}}} % indicator function
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\st}{\mbox{ s.t. }} % such that or subject to

% number sets
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}

% Calculus: Derivatives \& Integrals
\newcommand{\dm}[1]{\ensuremath{\,\mathrm{d}{#1}}} % Pretty symbol for differentials - ie, dx
\newcommand{\deriv}[2]{\frac{d #1}{d #2}}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\DD}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}
\newcommand{\Di}[2]{\frac{\partial ^i #1}{\partial #2 ^i}}
\newcommand{\evalat}[1]{\left.#1\right|}
\newcommand{\parderiv}[2]{\frac{\partial #1}{\partial{#2}}}
\newcommand{\parDeriv}[3]{\frac{\partial^{#3} #1}{\partial{#2}^{#3}}}
\newcommand{\parwrt}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\parpowrt}[2]{\frac{\partial^{#1}}{\partial {#2}^{#1}}}
\newcommand{\partwowrt}[2]{\frac{\partial^{2}}{\partial {#2} \partial{#1}}}

% basic linear algebra notation
\newcommand{\ones}{\mathop{\mathbf{1}}} % vector of ones
\newcommand{\diag}{\mathop{\mbox{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}} % null space ( range is \Range, above)
\newcommand{\Null}{\mathcal N} % null space ( range is \Range, above)
\newcommand{\Tr}{\textrm{Tr}} % trace
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}  % normroduct
\newcommand{\tp}[1]{\ensuremath{{#1}^\top}} % transpose with argument
\newcommand{\trp}{^{\mathrm{T}}} % Transpose
\newcommand{\itrp}{^{-\mathrm{T}}} % inverse-transpose
\newcommand{\inprod}[2]{\langle #1,#2\rangle}

% Probability notation
\newcommand{\pialg}{\pi\text{-algebra}}
\newcommand{\sigalg}{\sigma\text{-algebra}}
\newcommand{\alg}[1]{\mathcal{#1}} % sigma algebra notation
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Prob}[1]{\mathbb{P}\left[#1\right]}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\Norm}[2]{\mathcal{N}\left(#1, #2\right)} % normal distribution
%\newcommand{\mvn}[4]{\frac{1}{(2\pi)^{\frac{#4}{2}} |#3|^\frac{1}{2}} 
%\exp \left[-\tfrac{1}{2} (#1 - #2)\trp #3^{-1}(#1-#2)\right]} % multivariate normal
%% Notation for specific projects
%\newcommand{\mvnzero}[2]{\frac{1}{|2\pi #2|^\frac{1}{2}}
%\exp \left[-\tfrac{1}{2} #1\trp #2^{-1}#1\right]}  % zero-mean mvn


% matrix variables
\newcommand{\identityMat}{\ensuremath{I}}

\usepackage{forloop}
\newcommand{\defvec}[1]{\expandafter\newcommand\csname v#1\endcsname{{\mathbf{#1}}}}
\newcounter{ct}
\forLoop{1}{26}{ct}{
    \edef\letter{\alph{ct}}
    \expandafter\defvec\letter
}
\newcommand{\defmat}[1]{\expandafter\newcommand\csname m#1\endcsname{{\mathbf{#1}}}}
\forLoop{1}{26}{ct}{
    \edef\letter{\Alph{ct}}
    \expandafter\defmat\letter
}
\newcommand{\vmu}{\bm{\mu}}
\newcommand{\veta}{\bm{\eta}}
\newcommand{\vepsilon}{\bm{\epsilon}}
\newcommand{\vlambda}{\bm{\lambda}}


\newcommand{\mLambda}{\bm{\Lambda}}

% mutual information symbols (for MI estimation)
\newcommand{\nmax}{{n_{max}}}
\newcommand{\Dir}{\mathrm{Dir}}
\newcommand{\Snsb}{\hat S_{NSB}}
\newcommand{\Sdir}{\hat S_{Dir}}
\newcommand{\Sbls}{\hat S_{BLS}}
\newcommand{\Laplace}{\mathcal{L}} % laplace transform
\newcommand{\pnsb}{{p_{NSB}}}
\newcommand{\Ixy}{{I_{xy}}}

% convex analysis symbols (for optimization class)
\newcommand{\conv}{\text{conv}} % convex hull
\newcommand{\aff}{\text{Aff }} % affine hull
\newcommand{\extp}{\text{Ext}} %extreme points
%\newcommand{\argmin}{\mathrm{arg}\min}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\grad}{\nabla}
\newcommand{\curl}{\nabla\times}
\newcommand{\logdet}[1]{\log |#1|}


%% My own TheoremStyle
  \newtheoremstyle{evandefinition}{\topsep}{\topsep}%
     {}%         Body font  (\itshape)
     {}%         Indent amount (empty = no indent, \parindent = para indent)
     {\bfseries}% Thm head font
     {}%        Punctuation after thm head
     {\newline}%  Space after thm head  (default: 5pt plus 1pt minus 1pt)
     {\thmname{#1}\thmnumber{ #2}. \textit{\thmnote{ #3} }}%         Thm head spec


     \newtheoremstyle{indenteddefinition}{\topsep}{\topsep}
     {\addtolength{\leftskip}{2em}} %         Body font  (\itshape)
     {-1.75em}%         Indent amount (empty = no indent, \parindent = para indent)
     {\bfseries}% Thm head font % also: \scshape
     {}%        Punctuation after thm head
     { }%  Space after thm head  (default: 5pt plus 1pt minus 1pt)
     {\thmname{#1} \thmnumber{#2}. \textbf{(\thmnote{#3})}}%         Thm head spec
     % {} %         Thm head spec


% %% This code will allow me to have a bar around shit (uses ntheorem)
% %\theoremstyle{plain}
% \theorembodyfont{}
% \usepackage{color}
% \definecolor{gray}{rgb}{0.7,0.7,0.7}
% % This code turns the box around the theorem into a bar to the left
% \renewcommand*\FrameCommand{{\color{gray}\vrule width 1pt\hspace{10pt}}}


% general headings
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

\theoremstyle{evandefinition}
\newtheorem{definition}{Definition}
%\theoremstyle{definition}
% \theoremindent1em
% \theorembodyfont{\normalfont}
%\newframedtheorem{definition}{Definition}

\theoremstyle{indenteddefinition} 
\newtheorem{example}{Example}

\theoremstyle{remark} 
\newtheorem{exercise}{Exercise}
\newtheorem{remark}{Remark}

%% Make it so matrix has an align-column option ([c])
\makeatletter
\renewcommand*\env@matrix[1][c]{\hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols #1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Examples of things I might want to do.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
%%%%%%%%%%%%%%%%
%  Function with different cases:
%%%%%%%%%%%%%%%%
% \begin{align*}
%   q(\mu) &= \inf_x L(x,\mu)
% \\
% &=\left\{
% \begin{matrix}
% &c_0 + \mu c_1 - (b_0 - \mu b_1)^T ( A_0 + \mu A_1)^+ (b_0 + \mu
% b_1 )^T  &  A_0 + \mu A_1 \succeq 0,
% \\
% &\quad & b_0 + \mu b_1 \in \mathcal{R}(A_0 + \mu A_1)
% \\
% & \infty & \mathrm{otherwise}
% \end{matrix}\right.
% \end{align*}
% 

